SpatialVLA: Exploring Spatial Representations for Visual-Language-Action Model

In this paper, we claim that spatial understanding is the keypoint in robot manipulation, and propose SpatialVLA to explore effective spatial representations for the robot foundation model. Specifically, we introduce Ego3D Position Encoding to inject 3D information into the input observations of the visual-language-action model, and propose Adaptive Action Grids to represent spatial robot movement actions with adaptive discretized action grids, facilitating learning generalizable and transferrable spatial action knowledge for cross-robot control. SpatialVLA is first pre-trained on top of a vision-language model with 1.1 Million real-world robot episodes, to learn a generalist manipulation policy across multiple robot environments and tasks. After pre-training, SpatialVLA is directly applied to perform numerous tasks in a zero-shot manner. The superior results in both simulation and real-world robots demonstrate its advantage of inferring complex robot motion trajectories and its strong in-domain multi-task generalization ability. We further show the proposed Adaptive Action Grids offer a new and effective way to fine-tune the pre-trained SpatialVLA model for new simulation and real-world setups, where the pre-learned action grids are re-discretized to capture robot-specific spatial action movements of new setups. The superior results from extensive evaluations demonstrate the exceptional in-distribution generalization and out-of-distribution adaptation capability, highlighting the crucial benefit of the proposed spatial-aware representations for generalist robot policy learning. All the details and codes will be open-sourced.

==> rebuttal.tex <==
% \documentclass[conference]{IEEEtran}
% \input{preamble}
% \usepackage{times}
% \usepackage[numbers]{natbib}
% \usepackage{multicol}
% \usepackage{graphicx}
% \usepackage[bookmarks=true]{hyperref}
% \newcommand{\rssparagraph}[1]{{\bf #1.}}
% \begin{document}

    %%%%%%%% TITLE - PLEASE UPDATE
    \title{RSS Rebuttal of SpatialVLA [Paper-ID: 205]
    \vspace{-1cm}} % **** Enter the paper title and ID here
    \maketitle
    \thispagestyle{empty}
    \noindent
    [\textbf{\#ID:205}] We sincerely thank reviewer \textcolor{AC}{\#AC}, \textcolor{R1}{\#fSCZ},
    \textcolor{R2}{\#WYYj} and \textcolor{R3}{\#5n2s} for their thoughtful and
    constructive comments and suggestions. We have carefully revised our manuscript
    and summarized key revisions below to address their concerns.

    \boldparagraph{Q1.(\textcolor{AC}{\#all})}\textcolor{Q}{\textit{Advantage and limitation of spatial discretization?}}
    \noindent $\triangleright$Autoregressive paradigm with discretized action token has been widely adopted in existing VLAs~\citep{brohan2023rt,kim2024openvla,li2024cogact}, demonstrating significant advantages in large-scale training, seamless LLM integration, and instruction-following capabilities. The proposed Adaptive Action Grids adaptively align heterogeneous robotic actions to 3D space (\cref{fig:pipeline}), delivering notable strengths in efficient action representation (\cref{fig:bin}), fast token decoding (\cref{fig:teaser}), and flexible post-training transfer (\cref{sec:training}). 
    $\triangleright$\textit{A key concern is whether discretization limits precision.} As shown in \cref{tab:rebuttal_reso}, experiments across four grid resolutions demonstrate that performance improves from 1026 to 8194, but thereafter exhibits a gradual plateau or even a decline, beyond 6166. Notably, our method outperforms the 8196 uniform partitions \#1 $\mathcal{U}8196$ with only half partitions \#3 reso 4610, which is attributed to our \textit{adaptive grid partitioning strategy based on Gaussian probability density, allowing the model to concentrate on high-probability, fine-grained action spaces}, as depicted in~\cref{fig:bin}. Moreover, additional experiments in~\cref{fig:complex_task,tab:complex_task_real} show that \ours with discrete action space can handle fine-grained manipulation effectively. For the simplerenv~\cite{li24simpler} evaluation in~\cref{tab:rebuttal_simpler}, \ours also matches or outperforms the latest SOTA model $\pi_0$. $\triangleright$ However, \textit{higher-resolution or higher-dimensional action space introduces additional parameters to the 128k vocabulary, necessitating a trade-off between precision and efficiency}. The model may incur parameter overhead for humanoid robots with higher degrees of freedom. A flexible solution is to share action grids among embodiments like dexterous hands, bimanual arms, and legs, to be explored in future work.
    \begin{table}[htbp]
        \centering
        \setlength{\tabcolsep}{2pt}
        % \renewcommand{\arraystretch}{1.5}
        \vspace{-2ex}
        \caption{Action discretization ablations on simplerenv~\cite{li24simpler}.}
        \vspace{-2ex}
        \resizebox{1\columnwidth}{!}{
        \begin{tabular}{l|cc|cc|cc|cc}
            \hline
            \#setting             & \multicolumn{2}{c|}{pick coke can} & \multicolumn{2}{c|}{move near} & \multicolumn{2}{c|}{put carrot} & \multicolumn{2}{c}{put eggplant} \\
            \hline
                                  & aggregation                        & matching                       & aggregation                              & matching                                  & partial & success & partial & success \\
            $[1]$. $\mathcal{U}$8196 & 77.9\%                             & 28.0\%                         & 64.2\%                                   & 55.0\%                                    & 45.8\%  & 12.5\%  &  79.2\% & 54.2\%  \\
            $[2]$. reso 1026      & 74.4\%                             & 67.3\%                         & 59.1\%                                   & 54.2\%                                    & 45.8\%  & 25.0\%  & 66.7\%  & 54.2\%  \\
            $[3]$. reso 4610      & 76.7\%                             & 68.0\%                         & 69.8\%                                   & 79.2\%                                    & 41.7\%  & 33.3\%  & 83.3\%  & 75.0\%  \\
            $[4]$. reso 6166      & 80.9\%                             & 74.0\%                         & 74.0\%                                   & 79.2\%                                    & 41.7\%  & 33.3\%  & 95.8\%  & 87.5\%  \\
            $[5]$. reso 8194      & 81.6\%                             & 70.7\%                         & 79.2\%                                   & 85.4\%                                    & 41.7\%  & 33.3\%  & 91.7\%  & 87.5\%  \\
            \hline
        \end{tabular}
            } \label{tab:rebuttal_reso}
        \vspace{-2ex}
    \end{table}
    
    \boldparagraph{Q2.(\textcolor{AC}{\#all})}\textcolor{Q}{\textit{Handle more complex task beyond pick-and-place?}}
    \noindent
    $\triangleright$ To address reviewers' concerns on generalizability and fine-grained tasks, we evaluate \ours with four new dexterity tasks in~\cref{fig:complex_task,tab:complex_task_real}. \ours performs well even in complex fine-grained manipulation, significantly outperforming OpenVLA~\citep{o2024open} (72.7\% vs 54.5\%). As discussed earlier, this shows the action grid resolution is not a critical limiting factor, benefiting from its probability-adaptive grids.

    \begin{figure}[htbp]
        \vspace{-2ex}
        \begin{center}
            \includegraphics[trim=0.4ex 0 0 0, clip, width=1.0\linewidth]{figure/complex_task.pdf}
        \end{center}
        \vspace{-2ex}
        \caption{Fine-grained manipulation beyond pick-and-place.}
        \label{fig:complex_task}
        \vspace{-2ex}
    \end{figure}
    \boldparagraph{Q3.(\textcolor{AC}{\#all})}\textcolor{Q}{\textit{Comparison with the latest advanced models?}}
    \noindent
    $\triangleright$As suggested by the reviewers, we further compared our model with $\pi_0$ and $\pi_0$-fast in~\cref{tab:rebuttal_simpler}, masking the state input for fairness. Experiments show that our model performs comparably to $\pi_0$ and $\pi_0$-fast and even surpasses state-included $\pi_0$ in Google robot tasks (75.1\% vs 70.1\%).
    \begin{table}[t]
        \centering
        \setlength{\tabcolsep}{2pt}
        % \renewcommand{\arraystretch}{1.5}
        % \vspace{-2ex}
        \caption{Fine-grained manipulation and depth ablations.}
        \vspace{-2ex}
        \resizebox{1\columnwidth}{!}{
        \begin{tabular}{l|c|c|c|c|c}
            \hline
            \#setting ($\mathbf{D}$:depth)& clean table & push-T & insert charger & make tea & avg \\
            \hline
            OpenVLA~\citep{kim2024openvla}                   & 72.7\%     & 72.7\%       & 18.2\%          & 54.5\%             & 54.5\%  \\
            \ours w/o $\mathbf{D}$    & 63.6\%     & 54.5\%       & 9.1\%          & 54.5\%             & 45.4\%  \\
            \ours sensor $\mathbf{D}$ & 90.9\%     & 81.8\%       & 27.3\%          & 81.8\%             & 70.5\%  \\
            \ours zoe $\mathbf{D}$    & 90.9\%     & 90.9\%       & 27.3\%          & 81.8\%             & 72.7\%  \\
            \hline
        \end{tabular}
        } 
        \label{tab:complex_task_real}
        % \vspace{-5ex}
    \end{table}
    \begin{table}[t]
        \centering
        \setlength{\tabcolsep}{2pt}
        % \renewcommand{\arraystretch}{1.5}
        \vspace{-2ex}
        \caption{Comparison with latest models on simplerenv.}
        \vspace{-2ex}
        \resizebox{1\columnwidth}{!}{
        \begin{tabular}{l|c|c|c|c|c}
            \hline
            \#google robot                             & pick coke & move near  & open drawer & close drawer & avg    \\
            \hline
            OpenVLA~\citep{kim2024openvla}                                    & 16.3\%    & 46.2\%     & 19.4\%      & 51.8\%       & 27.7\% \\
            RoboVLM~\citep{li2023generalist}                                    & 77.3\%    & 61.7\%     & 33.3\%      & 53.1\%       & 63.4\% \\
            $\pi_{0}$~\cite{black2024pi_0} \textcolor{red}{w state}         & 88.0\%    & 80.3\%     & 66.7\%      & 45.2\%       & 70.1\% \\
            \ours                                      & 86.0\%    & 77.9\%     & 50.0\%      & 64.8\%       & 75.1\% \\
            \hline
            \#widowx                                   & put spoon & put carrot & stack block & put eggplant & avg    \\
            \hline
            OpenVLA~\citep{kim2024openvla}                                    & 2.05\%    & 16.7\%    & 6.3\%      & 6.2\%        & 7.8\%  \\
            RoboVLM~\citep{li2023generalist}                                    & 41.7\%    & 25.0\%     & 29.15\%     & 58.3\%       & 38.5\% \\
            % $\pi_{0}$-fast w/o state & 45.8\%        & 50.0\%         & 45.5\%          & 74.5\%           & 53.9\%      \\
            $\pi_{0}$-fast~\cite{black2024pi_0} \textcolor{blue}{w/o state} & 41.7\%    & 47.9\%     & 37.5\%      & 68.7\%       & 48.9\% \\
            $\pi_{0}$~\cite{black2024pi_0} \textcolor{blue}{w/o state}      & 35.4\%    & 47.4\%     & 45.0\%      & 56.2\%       & 46.0\% \\
            \ours                                      & 18.75\%   & 27.1\%     & 45.85\%     & 100\%        & 47.9\% \\
            \hline
        \end{tabular}
        } 
        \label{tab:rebuttal_simpler}
        \vspace{-5ex}
    \end{table}
    
    \boldparagraph{Q3.(\textcolor{R1}{\#fSCZ})}\textcolor{Q}{\textit{Complexity and noise analysis of ZoeDepth model?}}
    \noindent
    $\triangleright$ We must emphasize that ZoeDepth is used because depth is unavailable for all 28 datasets in OXE~\cite{o2024open} and RH20T~\cite{fang2023rh20t}. In pretraining, we utilize ZoeDepth to predict depth and ensure feasibility. In contrast, downstream fine-tuning allows for either ZoeDepth or sensor-captured depth in~\cref{tab:complex_task_real}. Visualization results show that \textit{sensor depth is noisy and disruptive, while ZoeDepth provides smoother inputs}. Our model with ZoeDepth achieves 72.7\% ACC, surpassing models with sensor depth (70.5\%) and without depth (45.4\%). This confirms the significant benefits of Ego3D PE with ZoeDepth, which \textit{captures relative spatial layouts, rendering precise scale unnecessary}. Notably, ZoeDepth remains fixed during training, occupying only 8.6\% of parameters and 0.06s per action time cost, making it an efficient solution. Additionally, Layer Norm and zero weight initialization of Ego3D PE help mitigate noise issues.
    \begin{figure}[htbp]
        \vspace{-2ex}
        \begin{center}
            \includegraphics[trim=0.4ex 0 0 0, clip, width=1\linewidth]{figure/depth.pdf}
        \end{center}
        \vspace{-2ex}
        \caption{Depth across sensor, Zoe, and L1 (avg$\le$0.2).}
        \label{fig:depth_noise}
        \vspace{-3ex}
    \end{figure}
    
    \boldparagraph{Q5.(\textcolor{R2}{\#WYYj})}\textcolor{Q}{\textit{Clarify LIBERO-Goal experiments results?}}
    \noindent
    $\triangleright$The performance gap with OpenVLA arises from dataset modifications, as OpenVLA filters zero or repeated actions. Retraining on the modified LIBERO-Goal dataset, our model achieves $80\pm0.6$\% vs OpenVLA's $79.2\pm1.0$\%. The gap with Octo may stem from action head design: diffusion-based methods better capture multimodality and overfit to specific data, potentially favoring smaller datasets like LIBERO.
    
    \boldparagraph{Q6.(\textcolor{AC}{\#all})}\textcolor{Q}{\textit{Improving paper organization and
    enhancing clarity}}.
    \noindent
    $\triangleright$ We have carefully revised our manuscript according to the reviewers's
    comments, including (1) clarifying VLMs' benefits conceptually, (2) adding
    color legends for \cref{fig:bin}c, (3) discussing action discretization works, (4) citing
    for critical statements, (5) simplifying video slides, and (6) fixing typos.


    
    %%%%%%%%% REFERENCES
    % {
    %   \small
    %   \bibliographystyle{plainnat}
    %   \bibliography{main}
    % }
    
% \end{document}

==> tables/franka_detailed_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
    []
    \centering
    \caption{Detailed Evaluation Results on Real-World Franka Robot}
    \label{tab:real-franka}
    \begin{tabular}{l|ll|cccc}
        \hline
        \multicolumn{1}{c|}{Category}           & \multicolumn{2}{c|}{Tasks}                                & Diffusion Policy & Octo            & OpenVLA         & SpatialVLA      \\
        \hline
        \multirow{6}{*}{Single-task}            & \multicolumn{2}{l|}{push the teapot handle aside}         & 72.72            & \textbf{100.00} & \textbf{100.00} & 81.81           \\
                                                & \multirow{2}{*}{place the white pot on the cutting board} & Grasped          & \textbf{81.81}  & 72.72           & 63.63          & 72.72           \\
                                                &                                                           & Success          & \textbf{72.72}  & 63.63           & 54.54          & \textbf{72.72}  \\
                                                & \multirow{2}{*}{put the banana in the basket}             & Grasped          & 72.72           & 0.00            & 81.81          & \textbf{100.00} \\
                                                &                                                           & Success          & 72.72           & 0.00            & 54.54          & \textbf{100.00} \\
                                                & \multicolumn{2}{l|}{close the drawer}                     & \textbf{100.00}  & \textbf{100.00} & 81.81           & 72.72           \\
        \hline
        \multirow{10}{*}{Instruction following} & put red cube on green car                                 & Grasped          & 18.18           & \textbf{63.63}  & 54.54          & \textbf{63.63}  \\
                                                &                                                           & Success          & 9.09            & \textbf{63.63}  & 54.54          & 54.54           \\
                                                & put green cube on green car                               & Grasped          & 0.00            & 0.00            & \textbf{54.54} & 45.45           \\
                                                &                                                           & Success          & 0.00            & 0.00            & 36.36          & \textbf{45.45}  \\
                                                & put blue cube on green car                                & Grasped          & 0.00            & 45.45           & 45.45          & \textbf{72.72}  \\
                                                &                                                           & Success          & 0.00            & 45.45           & 27.27          & \textbf{63.63}  \\
                                                & grasp the orange in the plate                             & Grasped          & 27.27           & \textbf{72.72}  & 36.36          & 63.63           \\
                                                &                                                           & Success          & 18.18           & \textbf{63.63}  & 27.27          & 54.54           \\
                                                & grasp the croissant in the plate                          & Grasped          & 27.27           & 27.27           & 45.45          & \textbf{54.54}  \\
                                                &                                                           & Success          & 9.09            & 18.18           & 36.36          & \textbf{54.54}  \\
        \hline
        \multirow{6}{*}{Multi-task}             & \multicolumn{2}{l|}{push the teapot handle aside}         & 18.18            & 27.27           & 54.54           & \textbf{63.63}  \\
                                                & \multirow{2}{*}{place the white pot on the cutting board} & Grasped          & 36.36           & 36.36           & \textbf{72.72} & 54.54           \\
                                                &                                                           & Success          & 27.27           & 36.36           & \textbf{54.54} & 36.36           \\
                                                & \multirow{2}{*}{put the banana in the basket}             & Grasped          & 27.27           & 45.45           & 81.81          & \textbf{81.81}  \\
                                                &                                                           & Success          & 27.27           & 36.36           & 63.63          & \textbf{81.81}  \\
                                                & \multicolumn{2}{l|}{close the drawer}                     & 27.27            & 27.27           & 36.36           & \textbf{45.45}  \\
        \hline
        \multirow{2}{*}{Spatial understanding}  & place plush toy closet to robot on car                    & Grasped          & 45.45           & 63.63           & 45.45          & \textbf{72.72}  \\
                                                &                                                           & Success          & 27.27           & 27.27           & 45.45          & \textbf{63.63}  \\
        \hline
    \end{tabular}
\end{table*}

==> tables/isaac_google_robot.tex <==
\begin{table}[tbp]
  \centering
  \scriptsize
  \resizebox{\linewidth}{!}{
    \begin{tabular}{llccccc}
      \toprule
      \multirow{3}{*}{\begin{tabular}[l]{@{}l@{}}Google Robot\\ Evaluation Setup\end{tabular}} &
      \multirow{3}{*}{Policy}                    &
      \multicolumn{4}{c}{Pick Coke Can}          &
      Move Near                                                                                                           \\ \cmidrule{3-7}
                                                 &
                                                 &
      \begin{tabular}[l]{@{}l@{}}Horizontal\\ Laying\end{tabular}                  &
      \begin{tabular}[l]{@{}l@{}}Vertical\\ Laying\end{tabular}                  &
      \begin{tabular}[l]{@{}l@{}}Standing\end{tabular}                  &
      \begin{tabular}[l]{@{}l@{}}Avg. Success\end{tabular}                  &
      \begin{tabular}[l]{@{}l@{}}Avg. Success\end{tabular}                                                                                           \\ \midrule
      \multirow{5}{*}{Real Eval}                 & RT-1 (Converged)               & 0.960 & 0.880 & 0.720 & 0.853 & 0.633 \\
                                                 & RT-1 ($15\%$)                  & 1.000 & 0.960 & 0.800 & 0.920 & 0.583 \\
                                                 & RT-1-X                         & 0.880 & 0.560 & 0.840 & 0.760 & 0.450 \\
                                                 & Octo-Base                      & 0.440 & 0.200 & 0.240 & 0.293 & 0.350 \\
                                                 & RT-1 (Begin)                   & 0.200 & 0.000 & 0.200 & 0.133 & 0.017 \\ \midrule
      \multirow{7}{*}{\begin{tabular}[l]{@{}l@{}}\ours Eval \\ (Isaac, Variant Aggre.) \end{tabular}} & RT-1 (Converged)               & 0.418 & 0.377 & 0.436 & 0.410 & 0.150 \\
                                                 & RT-1 ($15\%$)                  & 0.428 & 0.306 & 0.590 & 0.441 & 0.100 \\
                                                 & RT-1-X                         & 0.340 & 0.182 & 0.618 & 0.380 & 0.125 \\
                                                 & Octo-Base                      & 0.015 & 0.020 & 0.010 & 0.015 & 0.020 \\
                                                 & RT-1 (Begin)                   & 0.036 & 0.040 & 0.054 & 0.044 & 0.000 \\ \cmidrule{2-7}
                                                 & \textbf{MMRV}$\downarrow$      & 0.096 & 0.112 & 0.016 & 0.064 & 0.053 \\
                                                 & \textbf{Pearson $r$}$\uparrow$ & 0.961 & 0.949 & 0.989 & 0.973 & 0.865 \\
      \bottomrule
    \end{tabular}}
  \caption{Real-world and Isaac Sim evaluation results for the Google Robot setup. The findings on Isaac Sim are consistent with the findings on the SAPIEN simulator.}
  \vspace{-1.7em}
  \label{tab:simplerenv_bridge}
\end{table}




==> tables/task_design.tex <==
\begin{table}[t]
	\centering
	% \setlength{\tabcolsep}{2pt}
	% \renewcommand{\arraystretch}{0.8}
	\caption{\textbf{Task Design}.}
	\resizebox{1\columnwidth}{!}{
	\begin{tabular}{l|ll}
		\toprule Task Name         & Dimension & Details \\
		\midrule \texttt{make tea} &           &         \\
		\texttt{cube}              &           &         \\
		\texttt{plush toy}         &           &         \\
		\texttt{plush toy spatial} &           &         \\
		\texttt{drawer}            &           &         \\
		\bottomrule
	\end{tabular}
	} \label{tab:ablation_pretrain}
\end{table}


==> tables/temp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
    \centering
    \caption{Detailed Evaluation Results on Real-World Franka Robot}
    \label{tab:real-franka}
    \begin{tabular}{ccccccccccccccccccccccccc}
    \hline
    \multicolumn{1}{l|}{Category}              & \multicolumn{6}{l|}{Single-task}                                                                                                                                                                                                                                  & \multicolumn{10}{l|}{Instruction following}                                                                                                                                                                                                                                                                                                                                                                       & \multicolumn{6}{l|}{Multi-task}                                                                                                                                                                                                                      & \multicolumn{2}{l|}{Spatial understanding}                 \\ \cline{1-2} \cline{8-8} \cline{18-18} \cline{24-25} 
    \multicolumn{1}{l}{\multirow{2}{*}{Tasks}} & \multicolumn{1}{l}{\multirow{2}{*}{push the teapot handle aside}} & \multicolumn{2}{l}{place the white pot on the cutting board}              & \multicolumn{2}{l}{put the banana in the basket}          & \multicolumn{1}{l}{\multirow{2}{*}{close the drawer}} & \multicolumn{1}{l}{put red cube on green car} & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{put green cube on green car} & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{put blue cube on green car} & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{grasp the orange in the plate} & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{grasp the croissant in the plate} & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{\multirow{2}{*}{push the teapot handle aside}} & \multicolumn{2}{l}{place the white pot on the cutting board} & \multicolumn{2}{l}{put the banana in the basket}          & \multicolumn{1}{l}{\multirow{2}{*}{close the drawer}} & \multicolumn{2}{l}{place plush toy closet to robot on car} \\ \cline{8-8} \cline{24-24}
    \multicolumn{1}{l}{}                       & \multicolumn{1}{l}{}                                              & \multicolumn{1}{l}{Grasped}         & \multicolumn{1}{l}{Success}         & \multicolumn{1}{l}{Grasped} & \multicolumn{1}{l}{Success} & \multicolumn{1}{l}{}                                  & \multicolumn{1}{l}{Grasped}                   & \multicolumn{1}{l}{Success} & \multicolumn{1}{l}{Grasped}                     & \multicolumn{1}{l}{Success} & \multicolumn{1}{l}{Grasped}                    & \multicolumn{1}{l}{Success} & \multicolumn{1}{l}{Grasped}                       & \multicolumn{1}{l}{Success} & \multicolumn{1}{l}{Grasped}                          & \multicolumn{1}{l}{Success} & \multicolumn{1}{l}{}                                              & \multicolumn{1}{l}{Grasped}   & \multicolumn{1}{l}{Success}  & \multicolumn{1}{l}{Grasped} & \multicolumn{1}{l}{Success} & \multicolumn{1}{l}{}                                  & \multicolumn{1}{l}{Grasped}  & \multicolumn{1}{l}{Success} \\ \cline{1-2} \cline{8-8} \cline{18-18} \cline{24-25} 
    \multicolumn{1}{|c|}{Diffusion Policy}     & \multicolumn{1}{c|}{72.72}                                        & \multicolumn{1}{c|}{\textbf{81.81}} & \multicolumn{1}{c|}{\textbf{72.72}} & \multicolumn{1}{c|}{72.72}  & \multicolumn{1}{c|}{72.72}  & \multicolumn{1}{c|}{\textbf{100.00}}                  & \multicolumn{1}{c|}{18.18}                    & \multicolumn{1}{c|}{9.09}   & \multicolumn{1}{c|}{0.00}                       & \multicolumn{1}{c|}{0.00}   & \multicolumn{1}{c|}{0.00}                      & \multicolumn{1}{c|}{0.00}   & \multicolumn{1}{c|}{27.27}                        & \multicolumn{1}{c|}{18.18}  & \multicolumn{1}{c|}{27.27}                           & \multicolumn{1}{c|}{9.09}   & \multicolumn{1}{c|}{18.18}                                        & \multicolumn{1}{c|}{36.36}    & \multicolumn{1}{c|}{27.27}   & \multicolumn{1}{c|}{27.27}  & \multicolumn{1}{c|}{27.27}  & \multicolumn{1}{c|}{27.27}                            & \multicolumn{1}{c|}{45.45}   & 27.27                       \\ \cline{1-2} \cline{8-8} \cline{18-18} \cline{24-25} 
    Octo                                       & \textbf{100.00}                                                   & 72.72                               & 63.63                               & 0.00                        & 0.00                        & \textbf{100.00}                                       & \textbf{63.63}                                & \textbf{63.63}              & 0.00                                            & 0.00                        & 45.45                                          & 45.45                       & \textbf{72.72}                                    & \textbf{63.63}              & 27.27                                                & 18.18                       & 27.27                                                             & 36.36                         & 36.36                        & 45.45                       & 36.36                       & 27.27                                                 & 63.63                        & 27.27                       \\ \cline{1-2} \cline{8-8} \cline{18-18} \cline{24-25} 
    OpenVLA                                    & \textbf{100.00}                                                   & 63.63                               & 54.54                               & 81.81                       & 54.54                       & 81.81                                                 & 54.54                                         & 54.54                       & \textbf{54.54}                                  & 36.36                       & 45.45                                          & 27.27                       & 36.36                                             & 27.27                       & 45.45                                                & 36.36                       & 54.54                                                             & \textbf{72.72}                & \textbf{54.54}               & 81.81                       & 63.63                       & 36.36                                                 & 45.45                        & 45.45                       \\ \cline{1-2} \cline{8-8} \cline{18-18} \cline{24-25} 
    SpatialVLA                                 & 81.81                                                             & 72.72                               & \textbf{72.72}                      & \textbf{100.00}             & \textbf{100.00}             & 72.72                                                 & \textbf{63.63}                                & 54.54                       & 45.45                                           & \textbf{45.45}              & \textbf{72.72}                                 & \textbf{63.63}              & 63.63                                             & 54.54                       & \textbf{54.54}                                       & \textbf{54.54}              & \textbf{63.63}                                                    & 54.54                         & 36.36                        & \textbf{81.81}              & \textbf{81.81}              & \textbf{45.45}                                        & \textbf{72.72}               & \textbf{63.63}              \\ \cline{25-25} 
    \end{tabular}
    \end{table}

==> tables/widowx_detailed_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[t]
  \centering
  % \setlength{\tabcolsep}{2pt}
  % \renewcommand{\arraystretch}{0.8}
  \caption{Detailed Evaluation Results on Real-World WidowX Robot}
  \label{tab:widowx_raw} \resizebox{2\columnwidth}{!}{
  \begin{tabular}{l|ll|ccccc}
    \hline
    \multicolumn{1}{c|}{Category}           & \multicolumn{2}{c|}{Tasks}                                  & RT-1-X  & Octo-Base & RoboVLM & OpenVLA         & SpatialVLA(Ours) \\
    \hline
    Articulated manipulation                & \multicolumn{2}{l|}{Close the microwave}                    & 54.55   & 54.55     & 72.73   & \textbf{100.00} & \textbf{100.00}  \\
    \hline
    \multirow{3}{*}{Pick and place}         & \multicolumn{2}{l|}{Lift the red chili peper}               & 36.36   & 45.45     & 0.00    & \textbf{72.72}  & \textbf{72.72}   \\
                                            & \multirow{2}{*}{Put eggplant in the basket}                 & Grasped & 45.45     & 36.36   & 27.27           & 63.63           & \textbf{81.81} \\
                                            &                                                             & Success & 0.00      & 9.09    & 9.09            & 63.63           & \textbf{72.72} \\
    \hline
    \multirow{2}{*}{Color recognition}      & \multirow{2}{*}{Put purple cup on white plate}              & Grasped & 18.18     & 0.00    & 45.45           & \textbf{63.63}  & 54.54          \\
                                            &                                                             & Success & 9.09      & 0.00    & 27.27           & 18.18           & \textbf{45.45} \\
    \hline
    \multirow{12}{*}{Spatial understanding} & \multirow{2}{*}{Put cup on pink cloth (cup on stove)}       & Grasped & 18.18     & 18.18   & 27.27           & 36.36           & \textbf{81.81} \\
                                            &                                                             & Success & 18.18     & 9.09    & 18.18           & 36.36           & \textbf{81.81} \\
                                            & \multirow{2}{*}{Put cup on pink cloth (cup in sink)}        & Grasped & 9.09      & 27.27   & 18.18           & 63.63           & \textbf{90.90} \\
                                            &                                                             & Success & 0.00      & 18.18   & 9.09            & 54.54           & \textbf{90.90} \\
                                            & \multirow{2}{*}{Put cup on pink cloth (cup on stove block)} & Grasped & 18.18     & 9.09    & 9.09            & 36.36           & \textbf{81.81} \\
                                            &                                                             & Success & 9.09      & 9.09    & 0.00            & 27.27           & \textbf{72.72} \\
                                            & \multirow{2}{*}{Put cup on pink cloth (cup on bowl sink)}   & Grasped & 18.18     & 18.18   & 9.09            & 54.54           & \textbf{81.81} \\
                                            &                                                             & Success & 0.00      & 18.18   & 9.09            & 45.45           & \textbf{81.81} \\
                                            & \multirow{2}{*}{Put carrot on plate (plate in sink)}        & Grasped & 9.09      & 27.27   & 45.45           & \textbf{63.63}  & 54.54          \\
                                            &                                                             & Success & 9.09      & 0.00    & 27.27           & 18.18           & \textbf{45.45} \\
                                            & \multirow{2}{*}{Put carrot on plate (plate on pot sink)}    & Grasped & 9.09      & 18.18   & 9.09            & 54.54           & \textbf{72.72} \\
                                            &                                                             & Success & 0.00      & 9.09    & 0.00            & 54.54           & \textbf{63.63} \\
    \hline
  \end{tabular}
  }
\end{table*}
